General Matrix-Matrix Multiplication Using SIMD features of the PIII

Generalised matrix-matrix multiplication forms the kernel of many mathematical algorithms. A faster matrix-matrix multiply immediately benefits these algorithms. In this paper we implement efficient matrix multiplication for large matrices using the floating point Intel Pentium SIMD (Single Instruction Multiple Data) architecture. A description of the issues and our solution is presented, paying attention to all levels of the memory hierarchy. Our results demonstrate an average performance of 2.09 times faster than the leading public domain matrix-matrix multiply routines.

==> Makefile <==
#
# Makefile
# - for matrixmult paper
#
#

TEXT = matrixmult.tex abstract.tex intro.tex sgemm.tex \
	conclusion.tex
BIB  = ../papers.bib

all: matrixmult.dvi

.PHONY : matrixmult.dvi
matrixmult.dvi: 
	latex matrixmult.tex
	latex matrixmult.tex
	bibtex matrixmult
	latex matrixmult.tex


ps: matrixmult.dvi
	dvips -ta4 matrixmult.dvi -o matrixmult.ps

dummy:

tidy:
	rm -f *~ *.bak

clean: tidy
	rm -f *.aux *.log *.bbl *.blg

spotless: clean
	rm -f matrixmult.dvi matrixmult.ps


==> blocking.tex <==
\section{Blocking}
\label{Blocking}

In a matrix multiply each element of the result matrix is generated 
by a dot-product. A sequence of floating point numbers are 
multiplied and accumulated.  Each pair of numbers implies
two floating point operations, so
if we rely purely on main memory to supply values, we have an
upper bound of 200Mflops using a 100MHz bus. Pentiums 
with SIMD instructions can potentially execute at a Mflop rate 4
times their clock rate, which would use values at a faster rate than
the bus can provide them.
Our algorithm must take into account the availability of L0
(registers), L1 and L2 caches to overcome the limitations of deep
memory hierarchies. On the PIII the L1 data cache is 16Kb 2-way
set-associative with a 3 cycle latency to the
registers; L2 cache is a unified 512Kb 4-way set-associative with a
6 cycle latency \cite{greer:1997}. 

Both L1 and L2 caches
are write back which means writes go to cache and main memory is only updated
when an updated cache line is overwritten. 
For a detailed treatment of
caches the reader is referred to
Chapter 5 of \cite{hennessy:1996}.

The standard matrix-matrix multiply technique for deep memory hierarchy
machines (used in \cite{greer:1997,bilmes:1996,whaley:1997}) is 
matrix blocking. The concept is to break a large matrix-matrix
multiply into a series of smaller matrix multiplies where the data required
will fit entirely into cache. This is illustrated in Figure
\ref{f:blocking}. Let $A$ be a matrix of dimension $M \times K$ and $B$ be a
matrix of dimension $K \times N$. Then $C \longleftarrow A B$ is the $M \times
N$ result. If we cannot fit all of $A$, $B$ and $C$ 
into L1 cache simultaneously a
large time penalty will be incurred each time we fetch an element, 
either from L2 cache, or worse, from main memory.
\begin{figure}
\begin{center}
\input{figures/blocking.pstex_t}
\caption{Blocking matrix multiplies for improved memory efficiency.}
\label{f:blocking}
\end{center}
\end{figure}
The order in which each block multiply is done is one of the blocking 
parameters. Figure \ref{f:dumb} shows how we define the order of the loops.
During blocking the operation we are performing is 
equivalent to a matrix multiplication that operates on blocks instead of
individual elements. The standard matrix multiply has 2 loops that iterate
over the elements of $C$ and 1 loop to iterate along a row of 
$A$ and a column of $B$. This loop performs a dot product that computes one
element of the result matrix. We define the outer loop at a cache level to be 
whichever of the three necessary loops that contains the others nested within
it. The inner loop at a cache level is the most nested loop. 
\begin{figure}
\begin{center}
\begin{verbatim}
for (x = 0; x < m; x++) {           /* outer loop  */
    for (y = 0; y < n; y++) {       /* middle loop */
        for (z = 0; z < k; z++) {   /* inner loop  */
            c[x*n + y] += a[x*k + z]*b[z*n + y];
        }
    }
}
\end{verbatim}
\end{center}
\caption{Naive matrix multiply code showing the outer loop and the inner loop.}
\label{f:dumb}
\end{figure}
A clever ordering of these loops can take 
advantage of the particular cache architecture to 
obtain peak performance. 
Blocking can be made hierarchical with small blocks at the L0 register level 
and larger blocks for L1 and L2 cache levels.
Good register allocation is critical 
and depends mainly on the number of registers available.
Table \ref{t:params} summaries the parameters to consider for blocking.
\begin{table}
\begin{center}
\begin{tabular}{|l|p{8cm}|}
\hline
\emph{Parameter} & \emph{Description} \\
\hline
$M$ & Rows of $A$. Fixed. \\
$N$ & Columns of $B$. Fixed. \\
$K$ & Columns of $A$ and rows of $B$. Fixed. \\
$m$ & \# of rows to block from $A$ into L2.\\
$n$ & \# of columns to block from $B$ into L2.\\
$k$ & \# of columns from $A$ and rows from $B$ to block into L2,
$mk + kn + mn$ elements should fit into L2.\\
$\text{L2}_{\text{outer}}$ & Do we increment $x$ or $y$ or $z$ in the outer 
loop of $a_{x,y}b_{y,z}$.\\ 
$\text{L2}_{\text{inner}}$ & Do we increment $x$ or $y$ or $z$ in the inner loop of 
$a_{x,y}b_{y,z}$.\\
$m'$ & \# of rows to block from $a_{x,y}$ into L1.\\
$n'$ & \# of columns to block from $b_{y, z}$ into L1.\\
$k'$ & \# of columns from $A$ and rows from $B$ to block into L1, $m'k' + k'n' +
m'n'$ elements should fit into L1.\\
$\text{L1}_{\text{outer}}$ & Do we increment $x$ or $y$ or $z$ in the outer loop of 
            $a'_{x,y}b'_{y,z}$.\\ 
$\text{L1}_{\text{inner}}$ & Do we increment $x$ or $y$ or $z$ in the inner loop of 
            $a'_{x,y}b'_{y,z}$.\\
L0 & How do we allocate registers.\\
\hline
\end{tabular}
\caption{Summary of blocking parameters for a 2 level cache architecture.}
\label{t:params}
\end{center}
\end{table}


==> kni.tex <==
\section{Floating-Point SIMD}
\label{Floating-Point SIMD}

This section describes the algorithm for using the floating point 
SIMD instructions to perform matrix-matrix multiplication. Special attention is
paid to the blocking strategy applied. We start by describing
the floating point Intel SIMD architecture then we describe the algorithm 
beginning with register allocation and working up through L1 cache
and L2 cache organisation.

\subsection{Floating Point SIMD Pipeline}

There are 8 128-bit special \texttt{xmm} registers on which all the floating 
point SIMD instructions operate. The instructions in Table \ref{t:inst} are 
used at the lowest level to implement matrix-matrix
multiplication. The
\texttt{PS} suffix on most of the instructions indicates the operation is
on 4 single precision numbers in parallel. We know that the \emph{minimum}
time to fetch data is 3 cycles, which occurs when the data resides in L1
cache.
\begin{table}
\begin{center}
\begin{tabular}{|l|c|p{7cm}|}
\hline
\emph{Instruction} & \emph{Cycles} & \emph{Description} \\
\hline
\texttt{MULPS} & 5 & Multiply four floating point numbers. \\
\texttt{ADDPS} &  3 & Add four floating point numbers. \\
\texttt{MOVUPS} & $>$3 & Move four floating point numbers to memory.\\
\texttt{MOVAPS} & $>$3 & Same as \texttt{MOVUPS} but faster. Requires 128-bit 
 data alignment.\\
\texttt{SHUFPS} & 3 & Shuffle four floating point numbers around in registers.\\
\texttt{MOVHLPS} & 3 & Shuffle and copy the high pair of values to the low 
pair in a new register.\\
\texttt{MOVLHPS} & 3 & Shuffle and copy the low pair of values to the high 
pair in a new register.\\

\texttt{ADDSS} &  3 & Add the first floating point number only.\\
\texttt{MOVSS} & $>$3 & Move the first floating point number to memory.\\
\texttt{PREFETCHT0} & N/A & pre-fetch 32 bytes into L1 cache starting at
mem. Does not cause processor stalls.\\
\texttt{CPUID} & 1 & Report on the availability of SIMD instructions. \\
\hline
\end{tabular}
\end{center}
\caption{Summary of the floating point SIMD instructions used.}
\label{t:inst}
\end{table}
The Intel FPU pipeline is organised in such a way that one floating point 
instruction can be issued per cycle as 
long as multiplies are followed by an add
and there are no stalls due to register dependencies. 
Our experiments showed that code which interleaves 
\texttt{MULPS} and \texttt{ADDPS}
calls and has no dependencies shorter than the execution pipeline, achieves a 
CPI (cycles per instruction) of 1.3 or 1350 Mflops on a 450MHz CPU. 
This places an upper bound on the Mflops achievable by ignoring data
transfer.

\label{L0 Blocking}

The problem of how to supply data to the processor fast enough to keep it 
utilised is exacerbated by the four-fold parallelism. We have devised a scheme 
to minimise the ratio of memory accesses to floating point operations 
using two core strategies:
accumulate results for as long as possible to reduce write backs, and
re-use values in registers as much as possible.
The authors of \cite{greer:1997} used several dot-products 
simultaneously to achieve
this. The dot products generate:
\begin{equation}
C_{i,j} \leftarrow A_{i,1}B_{1,j} + A_{i,2}B_{2,j} + \ldots + A_{i,K}B_{K,j}. 
\end{equation}
We took the same approach and found by trial and error that the 
optimal number of dot-products to do simultaneously is 
5. 
Figure \ref{f:iter} shows 
how these 5 dot products progress. Each black circle represents an 
element in the current matrix block.  Each dashed square represents 
one floating point value in an \texttt{xmm} register. Thus 4 dotted 
squares together form one 128-bit \texttt{xmm} register.
\begin{figure}
\begin{center}
\input{figures/iter.pstex_t}
\caption{Allocation of \texttt{xmm} registers, showing progression of the dot
products which form the innermost loop of the algorithm.}
\label{f:iter}
\end{center}
\end{figure}
\texttt{xmm0} keeps the next 4 values from the
$a'$ row we are operating on. Two registers (\texttt{xmm1} and \texttt{xmm2}) 
alternately keep 4 values from each of the 5 columns of the $b'$ (L1 block),
we are operating on. The use of \texttt{xmm1} and \texttt{xmm2} in an
alternating fashion allows one register to be loading a value while the other is
involved in floating point operations. The remaining 5 registers accumulate the
results. Figure \ref{f:reg} shows 
the operations performed in one iteration of the innermost loop. It can be
seen that 8 floating point operations are done on 
each column from $b'$
in each iteration, giving a total of 40 flops per iteration.  This Figure also
represents the L0 block, the equivalent of a vector-matrix multiply of dimension
$1 \times 4 \times 5$. 
\begin{figure}
\begin{center}
\input{figures/reg.pstex_t}
\caption{Floating point operations performed in one iteration of the 
innermost loop.}
\label{f:reg}
\end{center}
\end{figure}
Loads of the $b'$ values 
are done with 3 or more cycles between the load and use. This
accounts for the 3 cycle latency between L1 cache and registers.
Loads from $a'$ are done once for the next
40 floating point operations with at least 3 cycles before
their first use. 
Three techniques used to improve pipeline performance are:
\begin{itemize}
\item The $b'$ block is buffered into an area of 
memory assumed to be in L1 cache constantly (this will be discussed further
in section \ref{L1 Blocking}). This has the further
advantage of reducing translation lookahead buffer misses
\cite{greer:1999}.
\item The $b'$ values in the buffer are all aligned on 128-bit boundaries
      to allow use of \texttt{MOVAPS} instead of the slower \texttt{MOVUPS} call (see Table \ref{t:inst}). 
\item The next 8 $a'$ values in the row are pre-cached into L1 cache using the 
\texttt{PREFETCHT0} command.  The placement of these commands was
done by trial and error as recommended by Intel \cite{intelopt:1999}.
\end{itemize}
Data shuffling must sometimes be done on 
the \texttt{xmm} registers to re-order the four floating point
values. This is required if the four results in a single register 
must be accumulated into one, or if the four results must be written back to
non-contiguous memory. Shuffling is an expensive operation.
The cost of these operations is minimised by
putting off the shuffling and write back for as long as possible using long
dot products. The length of the optimal dot product will be computed in the next
section.

\subsection{L1 Blocking}
\label{L1 Blocking}

The L1 data cache is 16Kb 2-way set associative. This means there are two 
banks of cache, each of which can hold 2048 single precision values 
in one cache bank. 
The line of the cache bank into which a value is inserted is determined 
by the least significant bits of its address. If that line in the cache 
is already used in
both banks, i.e. two values already share addresses with the same least
significant bits, then the value is loaded into a bank chosen at random.
We cannot assume 100\% utilisation of both cache banks for matrix data 
because at any one time there are intermediate variables, 
function parameters and old data in the cache over which we have no control.
It is safer to assume that we can partially utilise one bank with 
matrix data. We
do this by ensuring the matrix data has contiguous addresses so that 
every element has different least-significant bits, hence making sure no matrix
data overlaps in cache \cite{greer:1999}. 
There is still a small chance that some 
matrix data will be ejected if, for instance, there are 
two or more intermediate variables which map to the same
cache line as matrix data. The random replacement policy prevents
us from putting the matrix data into exclusively one bank, 
but we ensure that
we only use one of the two cache lines available for a particular address.

To hold just the $b'$ matrix in L1 permanently, with a bank 
utilisation of 83\% we have a maximum length of 341 for the columns of 
$b'$ before L1 cache fills up. After unrolling, the innermost loop 
computes 16 elements of the dot product. The best length of dot product is
therefore a multiple of 16, which we set to be 336. The utilisation factor 
is included because we found that trying to fill the cache bank 
to 100\% degrades 
performance. We chose 83\% on the ad hoc basis that it allows five 
columns of $b'$ and one row of $a'$ to fit into a single bank 
assuming there are no conflicts. Experiments confirmed this choice of
utilisation factor gives good results.
Since $b'$ is large $(336 \times 5)$ compared to $a'$ $(1 \times 336)$, $b'$ 
is buffered into L1 cache. We want to re-load $b'$ rarely, 
so $\text{L1}_{\text{outer}}$ as defined in Table \ref{t:inst} was
moved along 5 columns of $b'$ at a time. $\text{L1}_{\text{inner}}$ 
iterates over one row of $a$ at a time.  
This is shown in Figure \ref{f:l1block}. 
We rely on the pre-fetching rather than buffering to get the 
$a'$ values into L1 ahead of time. 
To summarise: $m'=1$, $n'=5$, 
$k'=336$,  $\text{L1}_{\text{inner}} = \text{rows of}~a$, $\text{L1}_{\text{outer}} = \text{columns of}~b$. 
\begin{figure}
\begin{center}
\input{figures/l1block.pstex_t}
\caption{L1 Blocking Scheme.}
\label{f:l1block}
\end{center}
\end{figure}

\subsection{L2 Blocking} 

Our experiments showed that including L2 blocking improved our performance by
about 16\% for square matrices over dimension 400. Below this size all matrix 
data fits into L2 cache. Re-ordering the L2 loops affects performance by
less than 5\%. Much greater gains are made from good L1 and L0 management.
The L2 blocking parameters were chosen to be:
$m=100$, $n=100$, $k=336$, $\text{L2}_{\text{inner}} = \text{columns of}~A \text{, rows of}~B$, $\text{L2}_{\text{outer}} = \text{columns of}~B$.


==> mathdefs.tex <==
\DeclareMathOperator{\TD}{TD}
\DeclareMathOperator{\VCdim}{VCdim}
\DeclareMathOperator{\GRADMDP}{GRADMDP}
\DeclareMathOperator{\GRADPOMDP}{GRADPOMDP}
\DeclareMathOperator{\LINESEARCH}{LINESEARCH}
\DeclareMathOperator{\REWARD}{REWARD}
\DeclareMathOperator{\VAL}{VAL}
\DeclareMathOperator{\GRAD}{GRAD}
\DeclareMathOperator{\CONJGRAD}{CONJGRAD}
\DeclareMathOperator{\er}{er}
\newcommand{\pt}{{\tilde p}}
\newcommand{\qt}{{\tilde q}}
\newcommand{\erh}{{\hat{\er}}}
\newcommand{\etah}{{\hat{\eta}}}
\newcommand{\dhat}{{\hat{d}}}
\newcommand{\h}{{\mathbold{h}}}
\newcommand{\Pb}{{\mathbold{P}}}
\newcommand{\scPb}{{\mathbold{\scriptstyle P}}}
\newcommand{\mathbold}[1]{\mbox{\boldmath $\bf#1$}}
\newcommand{\glossaryentry}[3]{\item[#1] #2 \hfill #3}
\renewcommand{\Box}{\square}
\renewcommand{\glossary}[2]{}
\def\addcontentsline#1#2#3{} 
\newtheorem{thm}{Theorem}
\newtheorem{exmp}{Example}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{corr}[thm]{Corollary}
\newtheorem{defn}{Definition}
\newcommand{\D}{{\cal D}}
\newcommand{\ie}{{\em i.e.\ }}
\newcommand{\etal}{{\em et.\ al.\ }}
\newcommand{\iid}{{i.i.d.\ }}
\newcommand{\norm}{{\|\cdot\|}}
\newcommand{\eg}{{\em e.g.\ }}
\newcommand{\cf}{{\em c.f.\ }}
\newcommand{\etc}{{\em etc}}
\newcommand{\comp}[2]{{#1\circ#2}}
\newcommand{\epspic}[2]{{\parbox{#1}{\epsfxsize=#1\epsfbox{#2}}}}
\renewcommand{\d}[2]{d_\nu\left(#1,#2\right)}
\newcommand{\rangel}[1]{\rangle_{#1}}
\newcommand{\E}{\mathbold{E}}
\newcommand{\HH}{{\mathbb H}}
\newcommand{\Hs}{{\HH_\sigma}}
\renewcommand{\H}{{\cal H}}
\newcommand{\XY}{{X\times Y}}
\newcommand{\VY}{{V\times Y}}
\newcommand{\de}{=}%%{{\,\,\,\,\overset{\text{def}}{=}\,\,\,\,}}
\renewcommand{\P}{{\cal P}}
\newcommand{\PP}{{\cal P}}
\newcommand{\Zm}{{\(X\timesY\)^m}}
\newcommand{\Zn}{{\(X\timesY\)^n}}
\newcommand{\Zmn}{{\(X\timesY\)^{(m,n)}}}
\newcommand{\Znm}{{\(X\timesY\)^{(n,m)}}}
\newcommand{\Ztmn}{{\(X\timesY\)^{(2m,n)}}}
\newcommand{\Gtmn}{{\Gamma_{(2m,n)}}}
\newcommand{\zmn}{{z^{(m,n)}}}
\newcommand{\znm}{{z^{(n,m)}}}
\newcommand{\z}{{\mathbold{z}}}
\newcommand{\f}{{\mathbold{f}}}
\newcommand{\g}{{\bf g}}
\newcommand{\w}{{\bf w}}
\newcommand{\x}{{\bf x}}
\newcommand{\y}{{\bf y}}
\newcommand{\B}{{\cal B}}
\newcommand{\Q}{{\cal Q}}
\newcommand{\Pm}{{P^m}}
\newcommand{\zb}{{\bold{z}}}
\newcommand{\zbh}{{\hat{\zb}}}
\newcommand{\zbv}{{\smash[b]{\vec{\zb}}}}
\newcommand{\zbvh}{\zbv} %%{\smash[b]{\hat{\vec{\zb}}}}}
\newcommand{\zh}{{\hat z}}
\newcommand{\xh}{{\hat x}}
\newcommand{\sh}{{\hat s}}
\newcommand{\Xhat}{{\hat X}}
\newcommand{\Shat}{{\hat S}}
\newcommand{\Ehat}{{\hat E}}
\newcommand{\qhat}{{\hat q}}
\newcommand{\yh}{{\hat y}}
\newcommand{\Phat}{{\hat \P}}
\newcommand{\Phihat}{{\hat \Phi}}
\newcommand{\Psihat}{{\hat \Psi}}
\newcommand{\Jt}{{\tilde{J}}}
\newcommand{\Vt}{{\tilde{V}}}
\newcommand{\Js}{{J^*}}
\newcommand{\nablat}{\nabla}
\newcommand{\Ph}{{\hat P}}
\newcommand{\zs}{{\z_\sigma}}
\newcommand{\zsw}{{\z_\sigma(1)}}
\newcommand{\zst}{{\z_\sigma(2)}}
\newcommand{\zsij}{{\z_{\sigma(ij)}}}
\newcommand{\fhat}{{\hat f}}
\newcommand{\ghat}{{\hat g}}
\newcommand{\Fhat}{{\hat \F}}
\newcommand{\rhat}{{\hat \rho}}
\newcommand{\Eh}{{\hat E}}
\newcommand{\bw}{{\bold{w}}}
\newcommand{\be}{\begin{equation*}}
\newcommand{\ee}{$$}
\newcommand{\ep}{{\varepsilon}}
\newcommand{\Z}{{\cal Z}}
\newcommand{\A}{{\cal A}}
\newcommand{\C}{{\cal C}}
\newcommand{\N}{{\cal N}}
\newcommand{\Nco}{{\N_\co}}
\newcommand{\M}{{\cal M}}
\newcommand{\F}{{\cal F}}
\newcommand{\G}{{\cal G}}
\newcommand{\T}{{\mathbb T}}
\newcommand{\U}{{\cal U}}
\newcommand{\V}{{\cal V}}
\newcommand{\Y}{{\cal Y}}
\newcommand{\calS}{{\cal S}}
\newcommand{\Ch}{{\hat \C}}
\newcommand{\rhol}{\rho_{\!_l}}
\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}
\newcommand{\Pv}{{\vec{P}}}
\newcommand{\xb}{{\bold{x}}}
\newcommand{\yb}{{\bold{y}}}
\newcommand{\wb}{{\bold{w}}}
\newcommand{\Deltabar}{{\overline\Delta}}
\newcommand{\Fbar}{{\overline\F}}
\newcommand{\Gbar}{{\overline\G}}
\newcommand{\Pbar}{{\bar{P}}}
\renewcommand{\hbar}{{\overline h}}
\newcommand{\dbar}{{d^*}}
\newcommand{\co}{{\text{\rm co}}}
\newcommand{\jon}{{\text{\rm jon}}}
\newcommand{\cdm}{{d_{\text{\rm CDM}}}}
\newcommand{\cdmhat}{{\hat{d}_{\text{\rm CDM}}}}
\newcommand{\cdmhathat}{{\tilde{d}_{\text{\rm CDM}}}}
\newcommand{\lin}{{\text{\rm lin}}}
\newcommand{\sign}{{\text{\rm sign}}}
\newcommand{\IID}{{\text{\rm IID}}}
\newcommand{\OTS}{{\text{\rm OTS}}}
\newcommand{\CDM}{{\text{\rm CDM}}}
\newcommand{\VC}{{\text{\rm VC}}}
\newcommand{\cobar}[1]{{\overline{\text{\rm co}\(#1\)}}}
\newcommand{\linbar}[1]{{\overline{\text{\rm lin}\(#1\)}}}
\newcommand{\Cbar}{{{\cal C}^*}}
\newcommand{\fbar}{{\bar f}}
\newcommand{\lbar}{{\bar l}}
\newcommand{\pibar}{{\bar \pi}}
\newcommand{\zv}{{\vec{z}}}
\newcommand{\gv}{{\vec{g}}}
\newcommand{\fv}{{\mathbold{f}}}
\newcommand{\lv}{{\vec l}}
\newcommand{\hv}{{\vec h}}
\newcommand{\xv}{{\mathbold{x}}}
\newcommand{\yv}{{\vec y}}
\newcommand{\wv}{{\mathbold{w}}}
\newcommand{\vv}{{\vec v}}
\newcommand{\av}{{\vec a}}
\newcommand{\Xv}{{\vec X}}
\newcommand{\pr}[3]{{{#1}_1#2\dots#2{#1}_{#3}}}
\newcommand{\iton}{{1\leq i\leq n}}
\newcommand{\prd}[4]{{{#1}_{#2}#3\dots#3{#1}_{#4}}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\Rn}{{\R^n}}
\newcommand{\Rpm}{{(\mathbb R^+)^{2m}}}
\newcommand{\Rptm}{{(\mathbb R^+)^{(2m,n)}}}
\newcommand{\dl}{{\mbox{\boldmath$d_{L^1}$}}}
\newcommand{\dimp}{{\mbox{dimp}}}
\newcommand{\argmin}{{\mbox{argmin}}}
\newcommand{\plus}{{\mbox{plus}}}
\newcommand{\minus}{{\mbox{minus}}}
\newcommand{\DKL}{{\mbox{DKL}}}
\newcommand{\WKS}{{\mbox{WKS}}}
\newcommand{\PKS}{{\mbox{PKS}}}
\newcommand{\ch}{{\large \chi}}
\newcommand{\SZ}{{\cal S}_Z}
\newcommand{\SP}{{\cal S}_\P}
\newcommand{\Tbar}{{\overline T}}
\newcommand{\Sbar}{{\overline S}}
\newcommand{\Xbar}{{\overline X}}
\newcommand{\Hbar}{{\overline \H}}
\newcommand{\bool}{{\{\pm 1\}}}
\newcommand{\zm}{{z^m}}
\newcommand{\Hns}{{\[\HH^n\]_\sigma}}
\newcommand{\Hsn}{{\[\HH_\sigma\]^n}}
\newcommand{\XVA}{X\stackrel{\F}{\rightarrow}V\stackrel{\G}{\rightarrow}A}
\newcommand{\XfVGY}{X\stackrel{f}{\rightarrow}V\stackrel{\G}{\rightarrow}Y}











==> results.tex <==
\section{Results}
\label{Results}

Timings were done by multiplying two matrices with dimensions up to
$M=N=K=600$ on a PIII 450MHz processor.
L1 and L2 caches were completely 
flushed between each run to avoid any advantages from residual elements of 
cached matrices. For matrices of dimension higher than 
40, our sgemm always beats the ATLAS SGEMM. Best performance is achieved 
at dimensions greater than 150. Below this size the overhead of 
setting up buffers is prohibitive. After size 100 we achieve an average of 
655Mflops and a peak of 736Mflops. Performance is 
better if buffering occurs on the matrix with
the largest non-common dimension since this buffer is loaded once into L1 
for many reads of the non-buffered matrix. 

Figure \ref{f:results} shows
a graph of \codename performance compared to ATLAS. 
Average results of
655Mflops continue up to the largest tested size of dimension 3000. The lower
line represents ATLAS performance. \codename is on average 1.8
times faster than ATLAS for matrices over dimension 40 and has a peak
performance 1.96 times faster than ATLAS. The peak occurs for dimension 336,
which matches the $k$ parameter, eliminating an L2 blocking loop and the use of
boundary cases in one dimension, while keeping the optimal dot product length.

\begin{figure}
\begin{center}
\includegraphics[scale=0.7]{figures/results.eps}
\caption{Mflops for square matrices}
\label{f:results}
\end{center}
\end{figure}

The relatively large variations in performance between consecutive matrix
dimensions arise for two reasons: 
boundary effects where we either cannot fill the $B$ buffer with 5 
columns or not having a multiple of 16 in the length of the dot products.
ATLAS avoids this fluctuation by having separate functions for each different
boundary size \cite{whaley:2000}. \codename uses several special cases to cope
with the case where $N/n'$ is not an integer, but currently ignores the
situation where $K/k'$ is not an integer by padding with zeros.

Intel have released optimized multiplication code for matrices up to 
dimension $6 \times 6$ square
\cite{AP-930}. This code runs at 633 Mflops. This assumes no
main memory accesses since the matrices are small, thus \codename has better
performance in a more difficult case. However, it should be noted that 
small matrix multiply code suffers from requiring a high 
proportion of shuffling to floating point operations.

To put these results in context the dumb matrix 
multiply implemented as shown in \ref{f:dumb} achieves an average of 50Mflops.
This is only 14\% of the ATLAS performance and 8\% of \codename performance.

